Probabilistic Decoupling of Labels in Classification

In this paper we develop a principled, probabilistic, unified approach to non-standard classification tasks, such as semi-supervised, positive-unlabelled, multi-positive-unlabelled and noisy-label learning. We train a classifier on the given labels to predict the label-distribution. We then infer the underlying class-distributions by variationally optimizing a model of label-class transitions.

==> math/print_math.tex <==
\clearpage
\section{Mathematical Notation}
\vspace{0.5cm}
\newboolean{showcode}
\setboolean{showcode}{true}

\newcommand{\showcode}[1]{
	\ifthenelse{\boolean{showcode}}{ {#1} }{}
}

\subsection*{Numbers and Arrays}





{
\def\arraystretch{1.5}
\begin{tabular}{p{2.5cm}p{3.8cm}p{11cm}}
	$\displaystyle a, \theta$           & \verb+a, \theta+           & A scalar (integer or real)                             \\
	$\displaystyle \va, \vtheta, \vone$ & \verb+\va, \vtheta, \vone+ & A vector                                               \\
	$\displaystyle \mA, \mTheta$        & \verb+\mA, \mTheta+        & A matrix                                               \\
	$\displaystyle \tA$                 & \verb+\tA+                 & A tensor                                               \\
	$\displaystyle \mI_n$               & \verb+\mI_n+               & Identity matrix with $n$ rows and $n$ columns          \\
	$\displaystyle \mI$                 & \verb+\mI+                 & Identity matrix with dimensionality implied by context \\
	$\displaystyle \ra$                 & \verb+\ra+                 & A scalar random variable                               \\
	$\displaystyle \rva$                & \verb+\rva+                & A vector-valued random variable                        \\
	$\displaystyle \rmA$                & \verb+\rmA+                & A matrix-valued random variable
\end{tabular}
}
\vspace{0.25cm}


\subsection*{Indexing}
{
\def\arraystretch{1.5}
\begin{tabular}{p{2cm}p{5.8cm}p{11cm}}
	$\displaystyle \eva_i, \evtheta_i$         & \verb+\eva_i, \evtheta_i+         & Element $i$ of vector $\va$                           \\
	$\displaystyle \eva_{-i}$                  & \verb+\eva_{-i}+                  & Element $n-i+1$ of vector $\va$ (-1 for last element) \\
	$\displaystyle \emA_{i,j}, \emTheta_{i,j}$ & \verb+\emA_{i,j}, \emTheta_{i,j}+ & Element $i, j$ of matrix                              \\
	$\displaystyle \mA_{i,:}, \emTheta_{i,:}$  & \verb+\mA_{i, :}, \emTheta_{i,:}+ & Row $i$ of matrix                                     \\
	$\displaystyle \mA_{:,i}, \emTheta_{:,i}$  & \verb+\mA_{:, i}, \emTheta_{:,i}+ & Column $i$ of matrix                                  \\
	$\displaystyle \etA_{i, j, k}$             & \verb+\etA_{i, j, k}+             & Element $(i, j, k)$ of a 3-D tensor                   \\
	$\displaystyle \tA_{:, :, i}$              & \verb+\tA_{:, :, i}+              & 2-D slice of a 3-D tensor                             \\
	$\displaystyle \erva_i$                    & \verb+\erva_i+                    & Element $i$ of the random vector                      \\
	$\displaystyle \ermA_i$                    & \verb+\ermA_i+                    & Element $i$ of the random matrix
\end{tabular}
}
\vspace{0.25cm}


\subsection*{Sets}
{
\def\arraystretch{1.5}
\begin{tabular}{p{2.5cm}p{3.8cm}p{11cm}}
	$\displaystyle \sA$                 & \verb+\sA+                & A set                                             \\
	$\displaystyle \R, \N, \Z, \Q$      & \verb+\R, \N, \Z, \Q+     & Standard sets                                     \\
	$\displaystyle \{0, 1\}$            & \verb+\{0, 1\}+           & The set containing 0 and 1                        \\
	$\displaystyle \{0, 1, \dots, n \}$ & \verb+\{0, 1, \dots, n\}+ & The set of all integers between $0$ and $n$       \\
	$\displaystyle [a, b]$              & \verb+[a, b]+             & The real interval including $a$ and $b$           \\
	$\displaystyle (a, b]$              & \verb+(a, b]+             & The real interval excluding $a$ but including $b$
\end{tabular}
\vspace{0.25cm}
}


\subsection*{Calculus}
\def\arraystretch{1.5}
\begin{tabular}{p{2.5cm}p{3.8cm}p{11cm}}
	$\displaystyle \diff[x]{y}$        & \verb+\diff[x]{y}+      & Derivative of $y$ with respect to $x$                      \\[2ex]
	$\displaystyle \pardiff[x]{y} $    & \verb+\pardiff[x]{y}+   & Partial derivative of $y$ with respect to $x$              \\
	$\displaystyle \gradient{x}y $     & \verb+\gradient{x}y+    & Gradient of $y$ with respect to $\vx$                      \\
	$\displaystyle \mdiff[\mX]y $      & \verb+\mdiff[\mX]y+     & Matrix derivatives of $y$ with respect to $\mX$            \\
	$\displaystyle \tdiff[\tX]y $      & \verb+\tdiff[\tX]y+     & Tensor containing derivatives of $y$ with respect to $\tX$ \\
	$\displaystyle \hess[\vx]f(\vx)$   & \verb+\hess[\vx]f(\vx)+ & The Hessian matrix of $f$ at input point $\vx$             \\
	$\displaystyle \int f(\vx) \d\vx $ & \verb+\int f(\vx)\d\vx+ & Definite integral over the entire domain of $\vx$
\end{tabular}
\vspace{0.25cm}

\subsection*{Probability and Information Theory}
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
	$\displaystyle P(\ra)$                                      & A probability distribution over a discrete variable                                                          \\
	$\displaystyle p(\ra)$                                      & A probability distribution over a continuous variable, or over a variable whose type has not been specified  \\
	$\displaystyle \ra \sim P$                                  & Random variable $\ra$ has distribution $P$                                                                   \\
	$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$                                                               \\
	$\displaystyle \var(f(x)) $                                 & Variance of $f(x)$ under $P(\rx)$                                                                            \\
	$\displaystyle \cov(f(x),g(x)) $                            & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$                                                               \\
	$\displaystyle H(\rx) $                                     & Shannon entropy of the random variable $\rx$                                                                 \\
	$\displaystyle \KL ( P \Vert Q ) $                          & Kullback-Leibler divergence of P and Q                                                                       \\
	$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$         & Gaussian distribution %
	over $\vx$ with mean $\vmu$ and covariance $\mSigma$
\end{tabular}
\vspace{0.25cm}

\subsection*{Functions}
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
	$\displaystyle f: \sA \rightarrow \sB$     & The function $f$ with domain $\sA$ and range $\sB$                                                                                \\
	$\displaystyle f \circ g $                 & Composition of the functions $f$ and $g$                                                                                          \\
	$\displaystyle f(\vx ; \vtheta) $          & A function of $\vx$ parametrized by $\vtheta$.	(Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation)  \\
	$\displaystyle \log x$                     & Natural logarithm of $x$                                                                                                          \\
	$\displaystyle \sigma(x)$                  & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$                                                                         \\
	$\displaystyle \zeta(x)$                   & Softplus, $\log(1 + \exp(x))$                                                                                                     \\
	$\displaystyle || \vx ||_p $               & $p$ norm of $\vx$                                                                                                                 \\
	$\displaystyle || \vx || $                 & $2$ norm of $\vx$                                                                                                                 \\
	$\displaystyle x^+$                        & Positive part of $x$, i.e., $\max(0,x)$                                                                                           \\
	$\displaystyle \vone_{\mathrm{condition}}$ & is 1 if the condition is true, 0 otherwise
\end{tabular}
\vspace{0.25cm}
